On the Transferability of VAE Embeddings using Relational Knowledge with Semi-Supervision

We propose a new model for relational VAE semi-supervision capable of balancing disentanglement and low complexity modelling of relations with different symbolic properties. We compare the relative benefits of relation-decoder complexity and latent space structure on both inductive and transductive transfer learning. Our results depict a complex picture where enforcing structure on semi-supervised representations can greatly improve zero-shot transductive transfer, but may be less favourable or even impact negatively the capacity for inductive transfer.

==> sections/apdx/further_results.tex <==
\newpage

\section{Additional Results}
\label{apdx:sec:further_results}



\begin{figure}
    \centering
    \includegraphics[width=1.\textwidth]{Assets/apdx/macro_excludedclasses_comparison_b4_d10.pdf}
    \caption{Transductive transfer results showing (\textbf{upper}) the $\textsf{isEqual}$ F1 scores on the \textit{held out} subset digit classes (indicated by the horizontal axis groupings); and (\textbf{lower}) $\Delta\%$ difference \wrt baseline F1 for each relation-decoder and context, with standard deviation in parentheses. Both results obtained with $\beta=4$ for the VAE.
    These results indicate that lower complexity decoders perform better at transductive transfer.}
    \label{fig:macro_excludedclasses_comparison}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=1.\textwidth]{Assets/apdx/macro_excludedclasses_comparison_b12_d1.pdf}
    \caption{Transductive transfer results showing (\textbf{upper}) the $\textsf{isEqual}$ F1 scores on the \textit{held out} subset digit classes (indicated by the horizontal axis groupings); and (\textbf{lower}) $\Delta\%$ difference \wrt baseline F1 for each relation-decoder and context, with standard deviation in parentheses. Both results obtained with $\beta=4$ for the VAE.
    These results indicate that lower complexity decoders perform better at transductive transfer.}
    \label{fig:macro_excludedclasses_comparison}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=1.\textwidth]{Assets/apdx/macro_excludedclasses_comparison_b12_d10.pdf}
    \caption{Transductive transfer results showing (\textbf{upper}) the $\textsf{isEqual}$ F1 scores on the \textit{held out} subset digit classes (indicated by the horizontal axis groupings); and (\textbf{lower}) $\Delta\%$ difference \wrt baseline F1 for each relation-decoder and context, with standard deviation in parentheses. Both results obtained with $\beta=4$ for the VAE.
    These results indicate that lower complexity decoders perform better at transductive transfer.}
    \label{fig:macro_excludedclasses_comparison}
\end{figure}

